Influence of Solvent Quality on Depletion Potentials in Colloid-Polymer Mixtures

As first explained by the classic Asakura-Oosawa (AO) model, effective attractive forces between colloidal particles induced by depletion of nonadsorbing polymers can drive demixing of colloid-polymer mixtures into colloid-rich and colloid-poor phases, with practical relevance for purification of water, stability of foods and pharmaceuticals, and macromolecular crowding in biological cells. By idealizing polymer coils as effective penetrable spheres, the AO model qualitatively captures the influence of polymer depletion on thermodynamic phase behavior of colloidal suspensions. In previous work, we extended the AO model to incorporate aspherical polymer conformations and showed that fluctuating shapes of random-walk coils can significantly modify depletion potentials [W. K. Lim and A. R. Denton, Soft Matter 12, 2247 (2016); J. Chem. Phys. 144, 024904 (2016)]. We further demonstrated that the shapes of polymers in crowded environments depend sensitively on solvent quality [W. J. Davis and A. R. Denton, J. Chem. Phys. 149, 124901 (2018)]. Here we apply Monte Carlo simulation to analyze the influence of solvent quality on depletion potentials in mixtures of hard sphere colloids and nonadsorbing polymer coils, modeled as ellipsoids whose principal radii fluctuate according to random-walk statistics. We consider both self-avoiding and non-self-avoiding random walks, corresponding to polymers in good and theta solvents, respectively. Our simulation results demonstrate that depletion of polymers of equal molecular weight induces much stronger attraction between colloids in good solvents than in theta solvents and confirm that depletion interactions are significantly influenced by aspherical polymer conformations.

==> makefile <==
# Makefile to compile latex files
#all:
#	latex $(DOC).tex;\
#	bibtex $(DOC);\
#	latex $(DOC).tex;\
#	latex $(DOC).tex;\
#	dvips -t letter $(DOC).dvi;\
#	ps2pdf $(DOC).ps;\
#	evince $(DOC).pdf

DOC = ao-jcp-final

all:
	latex $(DOC).tex;\
	bibtex $(DOC);\
	latex $(DOC).tex;\
	latex $(DOC).tex;\
 	dvipdf $(DOC).dvi;

nobib:
	latex $(DOC).tex;\
	dvips -t letter $(DOC).dvi;\
	ps2pdf $(DOC).ps;\
	evince $(DOC).pdf

pdf:
	pdflatex $(DOC).tex;\
	bibtex $(DOC).aux;\
	pdflatex $(DOC).tex;\
	pdflatex $(DOC).tex;\
	evince $(DOC).pdf

clean:
	rm -f $(DOC).aux $(DOC).bbl $(DOC).blg \
	$(DOC).dvi $(DOC).log $(DOC).pdf $(DOC).ps \
	$(DOC)Notes.bib

